Bringing Simulation and Observation Together to Better Understand the Intergalactic Medium

The methods by which one characterizes the distribution of matter in cosmological simulations is intrinsically different from how one performs the same task observationally. In this paper, we make substantial steps towards comparing simulations and observations of the intergalactic medium (IGM) in a more sensible way. We present a pipeline that generates and fits synthetic QSO absorption spectra using sight lines cast through a cosmological simulation, and simultaneously identifies structure by directly analyzing the variations in HI and OVI number density. We compare synthetic absorption spectra with a less observationally motivated, but more straightforward density threshold-based method for finding absorbers. Our efforts focus on HI and OVI to better characterize the warm/hot intergalactic medium, a subset of the IGM that is challenging to conclusively identify observationally. We find that the two methods trace roughly the same quantities of HI and OVI above observable column density limits, but the synthetic spectra typically identify more substructure in absorbers. We use both methods to characterize HI and OVI absorber properties. We find that both integrated and differential column density distributions from both methods generally agree with observations. The distribution of Doppler parameters between the two methods are similar for Lya and compare reasonably with observational results, but while the two methods agree with each other with OVI systems, they both are systematically different from observations. We find a strong correlation between OVI baryon fraction and OVI column density. We also discuss a possible bimodality in the temperature distribution of the gas traced by OVI.

==> apj-bib.tex <==

\bibliographystyle{apj}

\begin{thebibliography}{35}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[{Armstrong(1967)}]{armstrong1967}
Armstrong, B. 1967, Journal of Quantitative Spectroscopy and Radiative
  Transfer, 7, 61

\bibitem[{{Bristow} \& {Phillipps}(1994)}]{1994MNRAS.267...13B}
{Bristow}, P.~D. \& {Phillipps}, S. 1994, \mnras, 267, 13

\bibitem[{{Bryan} \& {Norman}(1997)}]{1997astro.ph.10187B}
{Bryan}, G.~L. \& {Norman}, M.~L. 1997, ArXiv Astrophysics e-prints

\bibitem[{{Cen} \& {Chisari}(2011)}]{2011ApJ...731...11C}
{Cen}, R. \& {Chisari}, N.~E. 2011, \apj, 731, 11

\bibitem[{{Cen} \& {Fang}(2006{\natexlab{a}})}]{2006ApJ...650..573C}
{Cen}, R. \& {Fang}, T. 2006{\natexlab{a}}, \apj, 650, 573

\bibitem[{{Cen} \& {Fang}(2006{\natexlab{b}})}]{cen2006}
---. 2006{\natexlab{b}}, \apj, 650, 573

\bibitem[{{Cen} \& {Ostriker}(1992)}]{1992ApJ...399L.113C}
{Cen}, R. \& {Ostriker}, J.~P. 1992, \apjl, 399, L113

\bibitem[{{Cen} \& {Ostriker}(1999)}]{1999ApJ...514....1C}
---. 1999, \apj, 514, 1

\bibitem[{{Danforth} \& {Shull}(2005)}]{2005ApJ...624..555D}
{Danforth}, C.~W. \& {Shull}, J.~M. 2005, \apj, 624, 555

\bibitem[{{Danforth} \& {Shull}(2008)}]{danforth2008}
---. 2008, \apj, 679, 194

\bibitem[{{Danforth} {et~al.}(2006){Danforth}, {Shull}, {Rosenberg}, \&
  {Stocke}}]{2006ApJ...640..716D}
{Danforth}, C.~W., {Shull}, J.~M., {Rosenberg}, J.~L., \& {Stocke}, J.~T. 2006,
  \apj, 640, 716

\bibitem[{{Danforth} {et~al.}(2010){Danforth}, {Stocke}, \&
  {Shull}}]{2010ApJ...710..613D}
{Danforth}, C.~W., {Stocke}, J.~T., \& {Shull}, J.~M. 2010, \apj, 710, 613

\bibitem[{{Dav{\'e}} {et~al.}(2001){Dav{\'e}}, {Cen}, {Ostriker}, {Bryan},
  {Hernquist}, {Katz}, {Weinberg}, {Norman}, \& {O'Shea}}]{2001ApJ...552..473D}
{Dav{\'e}}, R., {Cen}, R., {Ostriker}, J.~P., {Bryan}, G.~L., {Hernquist}, L.,
  {Katz}, N., {Weinberg}, D.~H., {Norman}, M.~L., \& {O'Shea}, B. 2001, \apj,
  552, 473

\bibitem[{{Dav{\'e}} {et~al.}(1999){Dav{\'e}}, {Hernquist}, {Katz}, \&
  {Weinberg}}]{1999ApJ...511..521D}
{Dav{\'e}}, R., {Hernquist}, L., {Katz}, N., \& {Weinberg}, D.~H. 1999, \apj,
  511, 521

\bibitem[{{Fang} \& {Bryan}(2001)}]{fang2001}
{Fang}, T. \& {Bryan}, G.~L. 2001, \apjl, 561, L31

\bibitem[{{Ferland} {et~al.}(1998){Ferland}, {Korista}, {Verner}, {Ferguson},
  {Kingdon}, \& {Verner}}]{1998PASP..110..761F}
{Ferland}, G.~J., {Korista}, K.~T., {Verner}, D.~A., {Ferguson}, J.~W.,
  {Kingdon}, J.~B., \& {Verner}, E.~M. 1998, \pasp, 110, 761

\bibitem[{{Fukugita} {et~al.}(1998){Fukugita}, {Hogan}, \&
  {Peebles}}]{1998ApJ...503..518F}
{Fukugita}, M., {Hogan}, C.~J., \& {Peebles}, P.~J.~E. 1998, \apj, 503, 518

\bibitem[{{Fukugita} \& {Peebles}(2004)}]{2004ApJ...616..643F}
{Fukugita}, M. \& {Peebles}, P.~J.~E. 2004, \apj, 616, 643

\bibitem[{Hopkins \& Beacom(2006)}]{0004-637X-651-1-142}
Hopkins, A.~M. \& Beacom, J.~F. 2006, The Astrophysical Journal, 651, 142

\bibitem[{{Norman} {et~al.}(2007){Norman}, {Bryan}, {Harkness}, {Bordner},
  {Reynolds}, {O'Shea}, \& {Wagner}}]{2007arXiv0705.1556N}
{Norman}, M.~L., {Bryan}, G.~L., {Harkness}, R., {Bordner}, J., {Reynolds}, D.,
  {O'Shea}, B., \& {Wagner}, R. 2007, ArXiv e-prints

\bibitem[{{Oppenheimer} \& {Dav{\'e}}(2009)}]{2009MNRAS.395.1875O}
{Oppenheimer}, B.~D. \& {Dav{\'e}}, R. 2009, \mnras, 395, 1875

\bibitem[{{Oppenheimer} {et~al.}(2009){Oppenheimer}, {Dav{\'e}}, \&
  {Finlator}}]{oppenheimer2009}
{Oppenheimer}, B.~D., {Dav{\'e}}, R., \& {Finlator}, K. 2009, \mnras, 396, 729

\bibitem[{{Oppenheimer} {et~al.}(2012){Oppenheimer}, {Dav{\'e}}, {Katz},
  {Kollmeier}, \& {Weinberg}}]{2012MNRAS.420..829O}
{Oppenheimer}, B.~D., {Dav{\'e}}, R., {Katz}, N., {Kollmeier}, J.~A., \&
  {Weinberg}, D.~H. 2012, \mnras, 420, 829

\bibitem[{{O'Shea} {et~al.}(2004){O'Shea}, {Bryan}, {Bordner}, {Norman},
  {Abel}, {Harkness}, \& {Kritsuk}}]{2004astro.ph..3044O}
{O'Shea}, B.~W., {Bryan}, G., {Bordner}, J., {Norman}, M.~L., {Abel}, T.,
  {Harkness}, R., \& {Kritsuk}, A. 2004, ArXiv Astrophysics e-prints

\bibitem[{{Persic} \& {Salucci}(1992)}]{1992MNRAS.258P..14P}
{Persic}, M. \& {Salucci}, P. 1992, \mnras, 258, 14P

\bibitem[{Savage {et~al.}(2014){Savage}, {Kim}, {Wakker}, {Keeney},{Shull},
  {Stocke}, \& {Green}}]{2014ApJS..212....8S}{Savage}, B.~D. and {Kim}, T.-S. and {Wakker}, B.~P. and {Keeney}, B. and 
        {Shull}, J.~M. and {Stocke}, J.~T. and {Green}, J.~C., \apj, 212, 8

\bibitem[{Shull {et~al.}(2012)Shull, Smith, \& Danforth}]{shull2012}
Shull, J.~M., Smith, B.~D., \& Danforth, C.~W. 2012, \apj, 759, 23

\bibitem[{{Smith} {et~al.}(2008){Smith}, {Sigurdsson}, \&
  {Abel}}]{2008MNRAS.385.1443S}
{Smith}, B., {Sigurdsson}, S., \& {Abel}, T. 2008, \mnras, 385, 1443

\bibitem[{{Smith} {et~al.}(2011){Smith}, {Hallman}, {Shull}, \&
  {O'Shea}}]{britton2011}
{Smith}, B.~D., {Hallman}, E.~J., {Shull}, J.~M., \& {O'Shea}, B.~W. 2011,
  \apj, 731, 6

\bibitem[{{Stocke} {et~al.}(2006){Stocke}, {Penton}, {Danforth}, {Shull},
  {Tumlinson}, \& {McLin}}]{stocke2006}
{Stocke}, J.~T., {Penton}, S.~V., {Danforth}, C.~W., {Shull}, J.~M.,
  {Tumlinson}, J., \& {McLin}, K.~M. 2006, \apj, 641, 217

\bibitem[{{Tepper-Garc{\'{\i}}a} {et~al.}(2011){Tepper-Garc{\'{\i}}a},
  {Richter}, {Schaye}, {Booth}, {Dalla Vecchia}, {Theuns}, \&
  {Wiersma}}]{teppergarcia2011}
{Tepper-Garc{\'{\i}}a}, T., {Richter}, P., {Schaye}, J., {Booth}, C.~M., {Dalla
  Vecchia}, C., {Theuns}, T., \& {Wiersma}, R.~P.~C. 2011, \mnras, 413, 190

\bibitem[{{Thom} \& {Chen}(2008{\natexlab{a}})}]{2008ApJS..179...37T}
{Thom}, C. \& {Chen}, H. 2008{\natexlab{a}}, \apjs, 179, 37

\bibitem[{{Thom} \& {Chen}(2008{\natexlab{b}})}]{2008ApJ...683...22T}
---. 2008{\natexlab{b}}, \apj, 683, 22

\bibitem[{{Tilton} {et~al.}(2012){Tilton}, {Danforth}, {Shull}, \&
  {Ross}}]{tilton2012}
{Tilton}, E.~M., {Danforth}, C.~W., {Shull}, J.~M., \& {Ross}, T.~L. 2012,
  \apj, 759, 112

\bibitem[{{Tripp} {et~al.}(2008){Tripp}, {Sembach}, {Bowen}, {Savage},
  {Jenkins}, {Lehner}, \& {Richter}}]{tripp2008}
{Tripp}, T.~M., {Sembach}, K.~R., {Bowen}, D.~V., {Savage}, B.~D., {Jenkins},
  E.~B., {Lehner}, N., \& {Richter}, P. 2008, \apjs, 177, 39

\bibitem[{{Turk} {et~al.}(2011){Turk}, {Smith}, {Oishi}, {Skory}, {Skillman},
  {Abel}, \& {Norman}}]{yt}
{Turk}, M.~J., {Smith}, B.~D., {Oishi}, J.~S., {Skory}, S., {Skillman}, S.~W.,
  {Abel}, T., \& {Norman}, M.~L. 2011, \apjs, 192, 9

\end{thebibliography}

